Feature learning in feature-sample networks using multi-objective optimization

Data and knowledge representation are fundamental concepts in machine learning. The quality of the representation impacts the performance of the learning model directly. Feature learning transforms or enhances raw data to structures that are effectively exploited by those models. In recent years, several works have been using complex networks for data representation and analysis. However, no feature learning method has been proposed for such category of techniques. Here, we present an unsupervised feature learning mechanism that works on datasets with binary features. First, the dataset is mapped into a feature--sample network. Then, a multi-objective optimization process selects a set of new vertices to produce an enhanced version of the network. The new features depend on a nonlinear function of a combination of preexisting features. Effectively, the process projects the input data into a higher-dimensional space. To solve the optimization problem, we design two metaheuristics based on the lexicographic genetic algorithm and the improved strength Pareto evolutionary algorithm (SPEA2). We show that the enhanced network contains more information and can be exploited to improve the performance of machine learning methods. The advantages and disadvantages of each optimization strategy are discussed.

==> reuters.tex <==
% Copyright 2017 © Filipe Verri
% vim: spell spelllang=en:

\subsection{Enhancement on semi-supervised classification of texts}

\todo{
  Apply the method in Reuters Dataset.  Show that the possible number of and-features
  is very high -- more than $2^{21000}$.  Maybe put some theoretical expected number
  based on the network sparsity. (I already have the math, just need to write it).
}


==> tables/new_classification,p=60.tex <==
Breast 2010 & $0.63 \pm 0.06$ & (1) & $0.62 \pm 0.06$ & (1) & $\mathbf{0.65 \pm 0.06}$ & (1)\\
Ecoli & $0.76 \pm 0.03$ & (4) & $0.76 \pm 0.03$ & (4) & $0.76 \pm 0.03$ & (11)\\
Glass & $0.66 \pm 0.05$ & (5) & $0.68 \pm 0.05$ & (7) & $\mathbf{0.69 \pm 0.06}$ & (7)\\
Wine & $0.92 \pm 0.02$ & (15) & $\mathbf{0.93 \pm 0.03}$ & (9) & $\mathbf{0.93 \pm 0.02}$ & (3)\\

